How Beginning Programmers and Code LLMs (Mis)read Each Other

Generative AI models, specifically large language models (LLMs), have made strides towards the long-standing goal of text-to-code generation. This progress has invited numerous studies of user interaction. However, less is known about the struggles and strategies of non-experts, for whom each step of the text-to-code problem presents challenges: describing their intent in natural language, evaluating the correctness of generated code, and editing prompts when the generated code is incorrect. This paper presents a large-scale controlled study of how 120 beginning coders across three academic institutions approach writing and editing prompts. A novel experimental design allows us to target specific steps in the text-to-code process and reveals that beginners struggle with writing and editing prompts, even for problems at their skill level and when correctness is automatically determined. Our mixed-methods evaluation provides insight into student processes and perceptions with key implications for non-expert Code LLM use within and outside of education.

==> figures/edits.tex <==
\begin{figure}[t]
\begin{subfigure}{0.465\textwidth}
\includegraphics[width=\textwidth]{images/first_last_quality.pdf}
\label{fig:first_last}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{images/second_last_quality.pdf}
\label{fig:second_to_last}
\end{subfigure}
\caption{Histograms of the 282 prompts which lead to successes after 2 or more attempts. These represent trends in how students edit prompts. The figure on the (left) shows the number of words changed between a first prompt and last prompt. The figure on the (right) shows the final change that produces a successful final prompt.}
\label{fig:upside_down}
\end{figure}

==> figures/interface.tex <==
\begin{figure}
\begin{subfigure}{0.6\textwidth}
%\includegraphics[width=\textwidth]{images/convert_blank.png}
\includegraphics[width=\textwidth]{images/exp-start.pdf}
\vspace{5ex}
\caption{An example task posed to a participant. The interface displays the function name and several input/output examples. Participants write and submit a description in the text box. During our study, 85\% of students who attempted this problem wrote a successful description after a single CS1 course.}
\label{fig:charlie_start}
\end{subfigure}
\hfill
\begin{subfigure}{0.35\textwidth}
%\includegraphics[width=\textwidth]{images/convert_fail.png}
\includegraphics[width=\textwidth]{images/exp-fail.pdf}
\caption{We run expert tests automatically and highlight tests that fail. Students are then able to either edit their description by pressing "Try Again" or move on to another problem.}
\label{fig:charlie_fail}
\end{subfigure}
\caption{The \textit{Charlie the Coding Cow} interface.}
\label{fig:charlie_screenshots}
\end{figure}


==> figures/summary-difficulty.tex <==
\begin{figure}

   \includegraphics[width=0.5\textwidth]{images/difficulty-by-type.pdf}

\caption{We ranked average problem difficulty by problem category both between the research team and students. Researchers ranked problems on a scale of 1 to 3. Student difficulty is represented by average student success rate. The Math and Conditional categories were equally challenging for researchers.}
\label{fig:difficulty}
\end{figure}
